Sunlight-heated refugia protect frogs from chytridiomycosis: a mathematical modelling study

The fungal disease Chytridiomycosis poses a threat to frog populations worldwide. It has driven over 90 amphibian species to extinction and severely affected hundreds more. Difficulties in disease management have shown a need for novel conservation approaches. We present a novel mathematical model for chytridiomycosis transmission in frogs that includes the natural history of infection, to test the hypothesis that sunlight-heated refugia reduce transmission. The model is fit using approximate Bayesian computation to experimental data where a cohort of frogs, a fixed subset of which had cleared a prior infection, were provided access to either sunlight-heated or shaded refugia. Using our model, we can estimate the extent to which prior chytridiomycosis infection protects against subsequent infection, and quantify the effect of sunlight-heating of refugia. Results estimate a 40% reduction in chytridiomycosis transmission when frogs have access to sunlight-heated refugia, compared to shaded refugia. This strongly supports the hypothesis that the sunlight-heated refugia reduce disease transmission. Frogs that were infected and recovered were estimated to have a reduction in susceptibility of approximately 97% compared to frogs with no prior infection. This research provides quantitative evidence supporting sunlight-heated refugia as an effective disease management tool for chytridiomycosis in frog populations. By estimating both the impact of refugia and the protective effects of prior infection, the model provides an evidence base for implementing sunlight-heated refugia as part of amphibian conservation strategies. This work represents an important first step in using mathematical modelling to inform policy on the design and implementation of habitat-based interventions to support amphibian population recovery and long-term sustainability.

==> tables/infection-state-timing.tex <==
\begin{tabularx}{0.8\linewidth}{ *{4}{C} }

\toprule

Infection states & Naïve ($k=U$) & Vaccinated ($k=V)$ & Parameter used \\ 

\midrule 

$I_{k,1}$ & 3.27 & 1.76 & 2.5 \\
$I_{k,2}$ & 4.87 & 4.29 & 4.5 \\

\bottomrule

\end{tabularx}
